Improving Document-Level Sentiment Analysis with User and Product Context

Past work that improves document-level sentiment analysis by encoding user and product information has been limited to considering only the text of the current review. We investigate incorporating additional review text available at the time of sentiment prediction that may prove meaningful for guiding prediction. Firstly, we incorporate all available historical review text belonging to the author of the review in question. Secondly, we investigate the inclusion of historical reviews associated with the current product (written by other users). We achieve this by explicitly storing representations of reviews written by the same user and about the same product and force the model to memorize all reviews for one particular user and product. Additionally, we drop the hierarchical architecture used in previous work to enable words in the text to directly attend to each other. Experiment results on IMDB, Yelp 2013 and Yelp 2014 datasets show improvement to state-of-the-art of more than 2 percentage points in the best case.

==> 2-related-work.tex <==
\section{Related Work}

Document-level sentiment analysis aims to predict sentiment polarity of text usually taking the form of a lengthy document. 
Sentiment analysis with user and product information \cite{tang-etal-2015-user-product} is a particular kind of sentiment classification task in which the corresponding user (or review author) and the product that was evaluated are taken into consideration when predicting sentiment polarity. 

Neural networks have been widely used in sentiment classification \cite{socher-etal-2013-recursive,kim-2014-convolutional,ibm_cnn,tang-etal-2015-document,wang2016attention}, most existing work focuses solely on the text itself, with \newcite{tang-etal-2015-user-product} were first to identify the importance of incorporating user and product information for sentiment classification. In their work, a CNN-based encoder was used to get document representation and user and product information are represented in both vector and matrix form, and injected in the word embedding layer and classification layer. Subsequently, many methods were proposed for the purpose of better capturing user preferences and product-specific sentiment. \newcite{chen-etal-2016-neural-sentiment} used an LSTM encoder to obtain the sentence-level representation before combining them into a document representation.
In their model, user and products are represented as vectors in the embedding matrix and user-product vectors are used to gather important information in both word and sentence-level through the attention mechanism. \newcite{ma-etal-2017-cascading} proposed a cascading multi-way attention to model the dependencies among user, product and review. \newcite{dou-2017-capturing,long-etal-2018-dual} adopted a memory network to capture user and product information. To alleviate the cold-start problems %that some users and products don't have enough reviews, 
\newcite{amplayo-etal-2018-cold} proposed to utilize similar user information when a given user's reviews are limited. Furthermore, \newcite{amplayo-2019-rethinking} proposed a novel model that represents users and products as chunk-wise importance weight matrices in order to improve the performance by reducing the number of parameters to be optimized.

Most aforementioned studies focus on better capturing the preferences from user and product, however they neglect to incorporate the reviews from the same user and product, although this information might be learned implicitly. But we think explicitly utilizing such extra context is helpful for sentiment classification.


==> 5-analysis.tex <==
\subsection{Analysis}
Besides, to study the effect of explicitly utilizing the representations of all reviews, we conduct experiments on Yelp-2013 to compare our model's performance with BERT without update on classification for samples whose user and product do not have many reviews in training set. Specifically, we filter out the samples in dev set of Yelp 2013 that the amount of the reviews of their attached user and product is higher than a particular threshold, in this paper we have three threshold: {40\%, 50\%, 60\%}, the \% stands for the proportion of the amount of average documents for one user in Yelp 2013. The results are shown in Table \ref{exp_res:filtered}. We can see that our model performs much better than the BERT without update when there are fewer reviews. In other words, if one user or product doesn't have many reviews, it's embedding that only be updated by gradient descent can't capture user preference well. By explicitly taking advantage of the other reviews, the user and product representations can better model their preferences.

\begin{table}[!htb]

  \centering
  \caption{Experimental Results on filtered Yelp-2013.}
    \input{tbl-04-sparse-results}
  \label{exp_res:filtered}%
\end{table}%
% \jf{The following should be considered:
% \begin{itemize}
%     \item All error analysis should be performed on the dev set
%     \item Is performance correlated with review length?
%     \item Manual analysis of 50 cases where the model  \textit{always} outperforms the w/o Update model over several (5?) runs (Jennifer)
%     \item Manual analysis of 50 cases where the model is still wrong (Jennifer)
% \end{itemize}
% }

==> old-tbl-03-results.tex <==
\begin{tabular}{lcccccccccccccccc}
    \toprule
     && \multicolumn{2}{c}{IMDB} && \multicolumn{2}{c}{Yelp-2013}  && \multicolumn{2}{c}{Yelp-2014} \\ [1ex]
    
     && Acc. (\%) & RMSE && Acc. (\%) & RMSE  && Acc. (\%) & RMSE   \\
     
    \midrule
    
    
   
    % \textsc{Majority}  && 19.6 & 2.495 && 41.1  & 1.060 && 39.2  & 1.097  \\
     \textsc{BERT vanilla} && 47.9$_\text{0.46}$ & 1.243$_\text{0.019}$ && 67.2$_\text{0.46}$  & 0.647$_\text{0.011}$ && 67.5$_\text{0.71}$  & 0.621$_\text{0.012}$ \\
    
    % imdb - V355, yelp-2013 0620-fff 99%, yelp-2014 V388
    \textsc{IUPC w/o Update} && 52.1$_\text{0.31}$ & 1.194$_\text{0.010}$ && 69.7$_\text{0.37}$  & 0.605$_\text{0.007}$ && 70.0$_\text{0.29}$  & 0.601$_\text{0.007}$ \\
    
     % imdb - V359, yelp-2013 weight-decay-0-eval_results_in_paper, yelp-2014 V378
    \textsc{IUPC} (our model) && 53.8$_\text{0.57}$ & \textbf{1.151$_\text{0.013}$} && \textbf{70.5$_\text{0.29}$}  & \textbf{0.589$_\text{0.004}$} && \textbf{71.2$_\text{0.26}$}  & \textbf{0.592$_\text{0.008}$} \\[1ex]
    \textsc{upnn}  && 43.5 & 1.602 && 59.6  & 0.784 && 60.8  & 0.764  \\
    
    \textsc{updmn} && 46.5 & 1.351 && 63.9  & 0.662 && 61.3  & 0.720  \\
    
    \textsc{nsc} && 53.3 & 1.281 && 65.0  & 0.692 && 66.7  & 0.654  \\
    
    \textsc{cma}   && 54.0 & 1.191 && 66.3  & 0.677 && 67.6  & 0.637  \\
    
    \textsc{dupmn} && 53.9 & 1.279 && 66.2  & 0.667 && 67.6  & 0.639  \\
    
    \textsc{hcsc}  && 54.2 & 1.213 && 65.7  & 0.660 && 67.6  & 0.639  \\
    
    \textsc{huapa} && 55.0 & 1.185 && 68.3  & 0.628 && 68.6  & 0.626  \\
    
    \textsc{chim}  && \textbf{56.4} & 1.161 && 67.8  & 0.641 && 69.2  & 0.622  \\
    
    \textsc{rrp-upm} && 56.2 & 1.174 && 69.0  & 0.629 && 69.1  & 0.621 \\
    
    
    
    \bottomrule
    \end{tabular}%

==> tbl-02-labels.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    Datasets & 1 & 2  & 3 & 4  & 5 & 6  & 7 & 8 & 9 & 10\\
    \hline
    IMDB & 2.75\% & 2.37\% & 3.51\% & 5.16\% & 8.33\% & 12.80\% & 19.11\% & 20.25\% & 12.37\% & 13.31\% \\
    \hline
    Yelp 2013 & 3.45\% & 8.29\% & 19.10\% & 41.58\% & 27.57\% & -  & - & - & - & -  \\
    \hline
        Yelp 2014 & 3.96\% & 8.84\% & 19.87\% & 39.69\% & 27.63\% & -  & - & - & - & -  \\
    \hline
\end{tabular}%

==> tbl-03-results-old.tex <==
\begin{tabular}{lcccccccccccccccc}
    \toprule
     && \multicolumn{2}{c}{IMDB} && \multicolumn{2}{c}{Yelp-2013}  && \multicolumn{2}{c}{Yelp-2014} \\ [1ex]
     && Acc. (\%) & RMSE && Acc. (\%) & RMSE  && Acc. (\%) & RMSE   \\
    \midrule
    % \textsc{Majority}  && 19.6 & 2.495 && 41.1  & 1.060 && 39.2  & 1.097  \\
     \textsc{BERT vanilla} && 47.9$_\text{0.46}$ & 1.243$_\text{0.019}$ && 67.2$_\text{0.46}$  & 0.647$_\text{0.011}$ && 67.5$_\text{0.71}$  & 0.621$_\text{0.012}$ \\
    
    % imdb - V355, yelp-2013 0620-fff 99%, yelp-2014 V388
    \textsc{IUPC w/o Update} && 52.1$_\text{0.31}$ & 1.194$_\text{0.010}$ && 69.7$_\text{0.37}$  & 0.605$_\text{0.007}$ && 70.0$_\text{0.29}$  & 0.601$_\text{0.007}$ \\
    
     % imdb - V359, yelp-2013 weight-decay-0-eval_results_in_paper, yelp-2014 V378
    \textsc{IUPC} (our model) && 53.8$_\text{0.57}$ & \textbf{1.151$_\text{0.013}$} && \textbf{70.5$_\text{0.29}$}  & \textbf{0.589$_\text{0.004}$} && \textbf{71.2$_\text{0.26}$}  & \textbf{0.592$_\text{0.008}$} \\[1ex]
    \textsc{upnn}  && 43.5 & 1.602 && 59.6  & 0.784 && 60.8  & 0.764  \\
    
    \textsc{updmn} && 46.5 & 1.351 && 63.9  & 0.662 && 61.3  & 0.720  \\
    
    \textsc{nsc} && 53.3 & 1.281 && 65.0  & 0.692 && 66.7  & 0.654  \\
    
    \textsc{cma}   && 54.0 & 1.191 && 66.3  & 0.677 && 67.6  & 0.637  \\
    
    \textsc{dupmn} && 53.9 & 1.279 && 66.2  & 0.667 && 67.6  & 0.639  \\
    
    \textsc{hcsc}  && 54.2 & 1.213 && 65.7  & 0.660 && 67.6  & 0.639  \\
    
    \textsc{huapa} && 55.0 & 1.185 && 68.3  & 0.628 && 68.6  & 0.626  \\
    
    \textsc{chim}  && \textbf{56.4} & 1.161 && 67.8  & 0.641 && 69.2  & 0.622  \\
    
    \textsc{rrp-upm} && 56.2 & 1.174 && 69.0  & 0.629 && 69.1  & 0.621 \\
    
    
    
    \bottomrule
    \end{tabular}%
